Using Machine Learning Methods for Automation of Size Grid Building and Management

Fashion apparel companies require planning for the next season, a year in advance for supply chain management. This study focuses on size selection decision making for Levi Strauss. Currently, the region and planning group level size grids are built and managed manually. The company suffers from the workload it creates for sizing, merchant and planning teams. This research is aiming to answer two research questions: "Which sizes should be available to the planners under each size grid name for the next season(s)?" and "Which sizes should be adopted for each planning group for the next season(s)?". We approach to the problem with a classification model, which is one of the popular models used in machine learning. With this research, a more automated process was created by using machine learning techniques. A decrease in workload of the teams in the company is expected after it is put into practice. Unlike many studies in the state of art for fashion and apparel industry, this study focuses on sizes where the stock keeping unit represents a product with a certain size.

==> master_thesis_up.tex <==

\newpage
\section*{Addendum to Master thesis}

\textbf{Name student:} Salim Yunus \\
\textbf{Name promoter:} Prof. Dries Benoit \\
\textbf{Thesis title:} Using Machine Learning Methods for Automation of Size Grid Building and Management\\

\vspace{2cm}

Date \textbf{pre-defense:} 31.03.2021\\
Name and signature of one of the members of the Examination Board, testifying successful participation in the pre-defenses:\\

\vspace{2cm}
Date \textbf{seminar 1:} 27.02.2020\\
Title seminar 1: Big Data and the End of Epidemiology\\

Signature of the promoter, testifying approval of and attendance of the seminar:\\

\vspace{2cm}
Date \textbf{seminar 2:} 19.02.2020\\
Title seminar 2: Machine Learning and Causal Inference: Tools for Data Science\\

Signature of the promoter, testifying approval of and attendance of the seminar:\\

\newpage

\textbf{Seminar 1 more details}\\
\textbf{Time:} 16:00 \\
\textbf{Speaker's Name:} Patrick Bossuyt (Professor of Clinical Epidemiology, University of Amsterdam\\
\textbf{Abstract:} The arrival of Big Data, in combination with the rise of Machine Learning and Artificial Intelligence, has encouraged some analysts to announce the end of theory and the demise of the traditional scientific method. By implication, that would be the end of epidemiology and biostatistics as we know it. In the Petabyte era, we are now able to analyze data without hypotheses about what it might show. In this presentation, we will analyze the birth and the development of “Big Data”. We will also study recent obituaries for “Big Data”, and what they imply. From there we analyze the claim that the traditional scientific methods have reached their limits and explore the implications of these developments for the practice, future and training in epidemiology and biostatistics.\\
\textbf{Location:} The faculty board meeting room: Room 40.02, S2, Campus Sterre\\

\textbf{Seminar 2 more details}\\
\textbf{Time:} 14:00\\
\textbf{Speaker's Name:} Dr. Karla Diaz-Ordaz, London School of Hygiene and Tropical Medicine \\
\textbf{Abstract:} Health data scientists and statisticians are often consulted by medical and policy decision makers evaluating the effects of medicines or social programmes (henceforth referred to as treatments), who need reliable evidence about the long-term causal effects of competing treatment strategies in key populations. Machine learning (ML) methods have received a lot of attention in recent years within the data science community, especially in settings with a large number of variables. However, causal effect estimation often involves counterfactuals, and prediction tools from the ML literature cannot be readily used for causal inference. In the last decade, major innovations have taken place incorporating supervised ML tools into estimators for causal parameters such as the average treatment effect (ATE). This holds the promise of attenuating model misspecification issues, and enhancing researchers knowledge with variable selection. In this talk, I will review some of these developments incorporating machine learning in the estimation of the ATE of a binary treatment, under the “no unobserved confounding” and positivity assumptions. In particular, I will illustrate (1) an ensemble machine learning algorithm known as Super Learner, for prediction and (2) estimation of ATE with machine learning approaches, such as targeted maximum likelihood estimation. Throughout, I will use as illustrative example the evaluation of cancer immunotherapy in Non-Small-Cell Lung Cancer patients, using electronic health records and tumour genomic data from a large USA cohort.\\
\textbf{Location:} De Krook, Miriam Makebaplein 1, 9000 Ghent, Room: De Blauwe Vogel\\
